SALD: Self-Referenced Advantage Learning for Diffusion Models

Recent work on language-model adaptation has shown that single models can obtain informative training signals by evaluating their behavior in demonstrationor feedback-augmented contexts, with the help of a teacher network, which is driven by the student's learned parameters. Inspired by this internal-reference principle, we investigate how diffusion models can identify self-referenced training signals without external demonstrations or teacher networks. We introduce SALD, a self-referenced training framework that evaluates each image-caption pair at two noise levels using the same model. The easier, lower-noise path is evaluated without gradient tracking to provide a reference, while the harder, higher-noise path provides the training gradient. Rather than directly distilling the easy-path prediction, SALD uses the difference between two path errors to adapt the hardpath objective. The proposed Advantage-Guided Diffusion (AGD) converts this relative error into a differentiable sample-level weight. Temporal Advantage Memory (TAM) accumulates relative difficulty across training and adapts the future gap between the two noise levels. Spectral Advantage Decomposition (SAD) further compares the residual power spectra of the two paths and constructs a differentiable, frequency-derived latent-element weight. All components share a single set of model parameters, requiring neither an external teacher network nor additional trainable parameters during training or inference, and no modification to the inference procedure. Experiments across multiple architectures and datasets demonstrate consistent improvements in generation quality, while component-wise ablations quantify the contributions of the proposed components.

==> sec/table2.tex <==
\begin{wraptable}{r}{0.7\linewidth}
\vspace{-4.5mm}
\centering
\Large
\caption{Quantitative results on ($512\times512$) large-scale datasets. Best values per metric are in \textcolor{blue}{Blue}.}
\label{tab:results_small}
\vspace{-1mm}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|l|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Params (B)}} & \multirow{2}{*}{\textbf{Method}} 
  & \multicolumn{3}{c|}{\textbf{COCO (2017)}} 
  & \multicolumn{3}{c}{\textbf{MultiGen-20M}} \\
\cmidrule(lr){4-6}\cmidrule(lr){7-9}
 & & & \textbf{FID}$\downarrow$ & \textbf{CLIP}$\uparrow$ & \textbf{LPIPS}$\downarrow$ 
  & \textbf{FID}$\downarrow$ & \textbf{CLIP}$\uparrow$ & \textbf{LPIPS}$\downarrow$ \\
\midrule

\multirow{5}{*}{\textbf{SANA 1.6}} & \multirow{5}{*}{1.6} & Base 
  &26.49 & 26.44 &0.7411 &26.44 &26.25 &0.7541 \\
 & & SpeeD 
  &25.38 & 26.83 & 0.7409 & 26.11 & 26.26 & 0.7558 \\
 & & SRA 
  &26.89 & 26.32 & 0.7461 & 26.05 & 25.89 & 0.7554 \\
 & & Temporal Diff  
  &26.36 & 26.87 & 0.7405 & 26.31 & 26.29 & 0.7539 \\
 & & \textbf{RAD} 
  &\textcolor{blue}{\textbf{22.76}} & \textcolor{blue}{\textbf{26.88}} &\textcolor{blue}{\textbf{0.7391}} 
  &\textcolor{blue}{\textbf{23.86}} & \textcolor{blue}{\textbf{26.29}} & \textcolor{blue}{\textbf{0.7533}} \\
\midrule

\multirow{5}{*}{\textbf{SANA 0.6}} & \multirow{5}{*}{0.6} & Base 
  &31.59 & 26.80 &0.7408 &31.93 &26.68 & 0.7495 \\
 & & SpeeD 
  &31.47 & \textcolor{blue}{\textbf{27.06}} & 0.7411 & 31.57 & 26.69 & 0.7485 \\
 & & SRA 
  &31.26 & 26.92 & 0.7397 & 31.63 & 26.56 & 0.7473 \\
 & & Temporal Diff  
  &31.28 & 27.03 & 0.7424 & 31.67 & 26.66 & 0.7498 \\
 & & \textbf{RAD} 
  &\textcolor{blue}{\textbf{29.31}} & \textcolor{blue}{\textbf{27.06}} & \textcolor{blue}{\textbf{0.7374}} 
  &\textcolor{blue}{\textbf{29.15}} & \textcolor{blue}{\textbf{26.69}} &\textcolor{blue}{\textbf{0.7472}} \\
\midrule

\multirow{5}{*}{\textbf{PixArt-$\Sigma$}} & \multirow{5}{*}{0.6} & Base 
  &29.26 & 25.82 &0.7653 & 31.62 & 25.83 & 0.7306 \\
 & & SpeeD 
  &29.25 & 25.80 &0.7533
  & 31.42 & 25.83 & \textcolor{blue}{\textbf{0.7292}} \\
 & & SRA 
  &29.21 & 25.88 & 0.7575 & 31.28 & 25.88 & 0.7297 \\
 & & Temporal Diff  
  &29.21 & 25.85 & 0.7594 & 31.31 & 25.41 & 0.7306 \\
 & & \textbf{RAD} 
  &\textcolor{blue}{\textbf{28.14}} & \textcolor{blue}{\textbf{26.00}} &  \textcolor{blue}{\textbf{0.7516}} 
  &\textcolor{blue}{\textbf{30.47}} & \textcolor{blue}{\textbf{25.93}} &\textcolor{blue}{\textbf{0.7292}} \\
\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{wraptable}

==> sec/xtra.tex <==
\section*{AI Use Statement}
We used generative AI tools solely for language refinement and grammar correction. All other aspects of this work, including the methodology, implementation, experiments, analysis, results, and manuscript content, were completed by the authors. The authors take full responsibility for the final content of the paper.



\section*{Ethics Statement}
This work does not involve human subjects, sensitive personal information, or private or proprietary data. All experiments are conducted using publicly available image-text datasets, including MultiGen-20M, COCO, Flickr8k, CUB-200-2011, Oxford 102 Flowers, MAGICK, and the DALL$\cdot$E 3 1M dataset, which are used solely for training and evaluating SALD and the corresponding baseline methods. Our approach does not require human annotations, human preference data, external teacher models, or additional human feedback during training. Instead, SALD constructs an internal reference from the same diffusion model using an easier noise level, thereby avoiding reliance on external supervision or preference-based feedback. We acknowledge that text-to-image generation models may be misused to produce misleading, inappropriate, or harmful visual content. We therefore encourage the responsible use of the proposed method and compliance with the licenses and usage policies of the underlying datasets and pretrained models, as well as adherence to the ICLR Code of Ethics and established responsible research practices.


\section*{Reproducibility Statement}
We provide detailed descriptions of the SALD framework, training objective, and optimization procedure in Sections~\ref{sec:problem} and~\ref{sec:experiments}, with additional implementation details in Appendix~\ref{sec:addi_res}. The appendix includes the backbone configurations, training and evaluation settings, wall-clock comparisons, inference-step analysis, extended training experiments, and qualitative results. We evaluate SALD across four backbone configurations, including SANA 0.6B, SANA 1.6B, PixArt-$\Sigma$, and FLUX.2-Klein base, using seven datasets at $512\times512$ and $1024\times1024$ resolutions. The training configuration specifies the optimizer, learning-rate schedule, mixed-precision setting, gradient clipping, number of training steps, and inference settings. We additionally report extended training results up to $100$k steps to examine convergence beyond the main training budget. These details are provided to facilitate the reproduction of our reported experiments and comparisons.
